Bitangents of real algebraic curves: signed count and constructions

We study real bitangents of real algebraic plane curves from two perspectives. We first show that there exists a signed count of such bitangents that only depends on the real topological type of the curve. From this follows that a generic real algebraic curve of even degree $d$ has at least $\frac{d(d-2)}{2}$ real bitangents. Next we explain how to locate (real) bitangents of a (real) perturbation of a multiple (real) conic in $\mathbb{C}P^2$. As main applications, we exhibit a real sextic with a total of $318$ real bitangents and 6 complex ones, and perform asymptotical constructions that give the best, to our knowledge, number of real bitangents of real algebraic plane curves of a given degree.

==> Signed.tex <==
\section{Preliminaries on the Hilbert schemes}\label{sec:hilb}

In this section we compute the various Hilbert schemes with up to two points that we need through out the paper. This include the Hilbert schemes of curves with some simple singularities, and smooth surfaces. To do this, we first compute some \textit{punctual} Hilbert schemes before computing all the needed Euler characteristic in Section \ref{sec-euler-characteristics-hilb-schemes}.

	
	\subsection{The plane}
	
	We work over the ring of formal series $\CC\xy$.
	
		\begin{prop}
		An ideal of length $\leqslant 3$ of $\CC\xy$ is one of the following:
			\begin{enumerate}[label=(\roman*)]
			\item if the length is $1$, then $I=(x,y)=\mfk$,
			\item if the length is $2$, then $I=(ax+by)$ for some $[a:b]\in\CC P^1$,
			\item if the length is $3$, then $I$ is either the ideal of the fat point $(x^2,xy,y^2)=\mfk^2$, or a curvilinear ideal $(f,\mfk^3)$, where $f$ is a polynomial of degree at most $2$ vanishing at $0$ which is non-singular point.
			\end{enumerate}
		\end{prop}
		
		\begin{prop}
		The punctual Hilbert scheme of the plane $\CC^2$ is isomorphic to the cone over a rational cubic curve: the subscheme corresponding to the curvilinear points is isomorphic to the total space of $\O(3)$, and it compactifies with the point corresponding to the fat point ideal.
		\end{prop}



	\subsection{Node : $A_1$}
	
		\subsubsection{Description of the complex Hilbert scheme.} We work over the ring of formal series $\CC\xy$. The singularity is locally given $xy=0$.
		
		\begin{prop}
		An ideal of length $\leqslant 3$ of $\CC\xy/(xy)$ is one of the following:
			\begin{enumerate}[label=(\roman*)]
			\item if the length is $1$, then $I=(x,y)=\mfk$,
			\item if the length is $2$, then $I=(ax+by)$ for some $[a:b]\in\CC P^1$,
			\item if the length is $3$, then $I=(x^3,y),(ax^2+by),(x^2,y^2),(ax+by^2),(x,y^3)$.
			\end{enumerate}
		\end{prop}
		
		
		
		\begin{prop}
		We have the following Hilbert schemes:
		\begin{enumerate}[label=(\roman*)]
			\item $\hilb^\CC_1(A_1)$ is a point,
			\item $\hilb^\CC_2(A_1)$ is isomorphic to $\CC P^1$,
			\item $\hilb^\CC_3(A_1)$ is isomorphic to the wedge of two copies of $\CC P^1$. The node corresponds to the ideal $(x^2,y^2,xy)$.
			\end{enumerate}
		\end{prop}
		
		\begin{coro}
		We have the following generating series for the Euler characteristic of the punctual Hilbert schemes:
		$$e^\CC(A_1)=1+q+2q^2+3q^3+O(q^4).$$
		\end{coro}
		
		\begin{rem}
		More generally, the $n$-points Hilbert scheme of the $A_1$ singularity is a chain of $n$ spheres.
		\end{rem}
		
		
		\subsubsection{Real Hilbert schemes.} Over the reals, there are two types of $A_1$ singularities, known as elliptic and hyperbolic nodes:
		$$A^+_1: x^2+y^2=0 \text{ and }A^-_1: x^2-y^2=0.$$
		These arise from the two real structures it is possible to put on the $A_1$ singularity: the one that exchanges the two branches and the other. The involution induces an involution on the complex Hilbert scheme. To get the real Hilbert scheme, we need to look for the locus fixed by this involution.
		
		\begin{prop}
		We have the following Hilbert schemes for the $A^+_1$ singularity:
		\begin{enumerate}[label=(\roman*)]
			\item $\hilb^\RR_1(A^+_1)$ is a point,
			\item $\hilb^\RR_2(A^+_1)$ is isomorphic to $S^1$,
			\item $\hilb^\RR_3(A^+_1)$ is a point corresponding to the ideal $(x^2,y^2,xy)$.
			\end{enumerate}
		We have the following Hilbert schemes for the $A^-_1$ singularity:
		\begin{enumerate}[label=(\roman*)]
			\item $\hilb^\RR_1(A^-_1)$ is a point,
			\item $\hilb^\RR_2(A^-_1)$ is isomorphic to $\RR P^1$,
			\item $\hilb^\RR_3(A^-_1)$ is isomorphic to the wedge of two copies of $\RR P^1$. The node corresponds to the ideal $(x^2,y^2,xy)$.
			\end{enumerate}
		\end{prop}
		
		\begin{coro}
		We have the following generating series for the Euler characteristic of the punctual Hilbert schemes:
		\begin{align*}
		e^\RR(A_1^+)= & 1+q+q^3+O(q^4), \\
		e^\RR(A_1^-)= & 1+q-q^3+O(q^4). \\
		\end{align*}
		\end{coro}
	
	
	
	
	
	\subsection{Cusp : $A_2$}
	
		\subsubsection{Description of the complex Hilbert scheme.} We work over the ring of formal series $\CC\xy$. The singularity is locally given $x^2-y^3=0$.
		
		\begin{prop}
		An ideal of length $\leqslant 3$ of $\CC\xy/(x^2-y^3)$ is one of the following:
			\begin{enumerate}[label=(\roman*)]
			\item if the length is $1$, then $I=(x,y)=\mfk$,
			\item if the length is $2$, then $I=(x,y^2),(ax+by),(x^2,y)$ for some $[a:b]\in\CC P^1$,
			\item if the length is $3$, then $I=(x,y^3),(x^2,y^2),(ax+by^2)$.
			\end{enumerate}
		\end{prop}
		
		\begin{prop}
		We have the following Hilbert schemes:
		\begin{enumerate}[label=(\roman*)]
			\item $\hilb^\CC_1(A_2)$ is a point,
			\item $\hilb^\CC_2(A_2)$ is isomorphic to $\CC P^1$,
			\item $\hilb^\CC_3(A_2)$ is isomorphic to $\CC P^1$.
			\end{enumerate}
		\end{prop}
		
		\begin{coro}
		We have the following:
		$$e^\CC(A_2)=1+q+2q^2+2q^3+O(q^4).$$
		\end{coro}
		
		
		\subsubsection{Real Hilbert schemes.} There is a unique real structure on the $A_2$ singularity.
		
		\begin{prop}
		We have the following Hilbert schemes:
		\begin{enumerate}[label=(\roman*)]
			\item $\hilb^\RR_1(A_2)$ is a point,
			\item $\hilb^\RR_2(A_2)$ is isomorphic to $\RR P^1$,
			\item $\hilb^\RR_3(A_2)$ is isomorphic to $\RR P^1$.
			\end{enumerate}
		\end{prop}
		
		\begin{coro}
		We have the following:
		$$e^\RR(A_2)=1+q+O(q^4).$$
		\end{coro}
		
		
	
	



	\subsection{Euler characteristics of Hilbert schemes}
	\label{sec-euler-characteristics-hilb-schemes}
	
	We now gather the punctual Hilbert schemes to compute the Euler characteristics of the Hilbert scheme of a curve that present some singularities.
		
		\begin{lem}
		We have
		\begin{align*}
		e^\CC(C_0) = & (1-q)^{a} \\
		 = & 1-aq+\bino{a}{2}q^2-\bino{a}{3}q^3 +O(q^4) , \\
		e^\RR(C_0) = & (1-q^2)^{a/2} \\
		= & 1-\frac{a}{2}q^2 +O(q^4). \\
		\end{align*}
		\end{lem}
		
		\begin{proof}
		The first identity is known as the MacDonald formula, and comes from the fact that the Hilbert scheme of a smooth curve is just its symmetric power: $C_0^{[n]}=C_0^{(n)}$, \textit{i.e.} the choice of length $n$ subscheme of $C_0$ amounts to choose a symmetric configuration of $n$ points on $C_0$. For the real version of the MacDonald formula, this symmetric configuration needs to be invariant by the complex conjugation, so $n$ decomposes as $r+2s$ with $r$ being the number of real points and $s$ the number of pairs of complex conjugate points. As $\chi(\RR C_0)=0$, we get the result.
		\end{proof}
	
	We now care about giving an expression for the Euler characteristics of the Hilbert schemes of singular curves, relating them to the case of a smooth deformation of the curve. 
	
		\begin{lem}[($A_1$-curves)]
		Let $C_1$ be a curve with a node as unique singularity. Let $C_1^+$ (resp. $C_1^-$) be a real curve with an elliptic (resp. hyperbolic). We assume that a deformation of the curve has Euler characteristic $-a$. We have the following:
		\begin{align*}
		e^\CC(C_1) = & (1-q)^a\left( 1 + q +2q^2+3q^3 +O(q^4) \right)  \\
		e^\RR(C_1^+) = & (1-q^2)^{a/2} \left( 1+q+q^3 + O(q^4) \right) \\
		e^\RR(C_1^-) = & (1-q^2)^{a/2} \left( 1-q-q^3 + O(q^4) \right) \\
		\end{align*}
		\end{lem}
		
		\begin{lem}[($A_2$-curves)]
		We have the following:
		\begin{align*}
		e^\CC(C_2) = & (1-q)^a(1+2q+4q^2+6q^3+O(q^4)) \\
		e^\RR(C_2) = & (1-q^2)^{a/2}\left( 1 + O(q^4) \right) \\
		\end{align*}
		\end{lem}
	
		\begin{lem}[($A_1A_1$-curves)]
		We have the following:
		\begin{align*}
		e^\CC(C_{11}) = & (1-q)^a\left( 1+2q+5q^2+10q^3+O(q^4) \right) \\
		e^\RR(C_{11}^{++}) = & (1-q^2)^{a/2}\left(1+2q+q^2+2q^3   +O(q^4)\right) \\
		e^\RR(C_{11}^{+-}) = & (1-q^2)^{a/2}\left(1 -q^2 +O(q^4)\right) \\
		e^\RR(C_{11}^{--}) = & (1-q^2)^{a/2}\left(1 -2q+q^2-2q^3   +O(q^4)\right) \\
		e^\RR(C_{11}^{oo}) = & (1-q^2)^{a/2}\left(1+q^2+O(q^4)\right) \\
		\end{align*}
		\end{lem}
	
		\begin{lem}[($A_1A_2$-curves)]
		We have the following:
		\begin{align*}
		e^\CC(C_{12}) = & (1-q)^a\left( 1+3q+8q^2+17q^3+O(q^4) \right) \\
		e^\RR(C_{12}^+) = & (1-q^2)^{a/2}\left( 1+q+q^3+O(q^4) \right) \\
		e^\RR(C_{12}^-) = & (1-q^2)^{a/2} \left( 1-q-q^3+O(q^4) \right) \\
		\end{align*}
		\end{lem}
	
		\begin{lem}[($A_3$-curves)]
		We have the following:
		\begin{align*}
		e^\CC(C_3) = & (1-q)^a \left( 1+3q+7q^2+13q^3 +O(q^4) \right) \\
		e^\RR(C_3^+) = & (1-q^2)^{a/2} \left( 1+q+q^2+q^3 +O(q^4) \right) \\
		e^\RR(C_3^-) = & (1-q^2)^{a/2}\left( 1-q+q^2-q^3+O(q^4)\right) \\
		\end{align*}
		\end{lem}
		
		\begin{lem}[($A_1A_1A_1$-curves)]
		We have the following:
		\begin{align*}
		e^\CC(C_{111}) = & (1-q)^a\left( 1+ 3q+9q^2+22q^3 +O(q^4) \right) \\
		e^\RR(C_{111}^{+++}) = & (1-q^2)^{a/2}\left(1+3q+3q^2+4q^3  +O(q^4)\right) \\
		e^\RR(C_{111}^{++-}) = & (1-q^2)^{a/2}\left(1+q-q^2 +O(q^4)\right) \\
		e^\RR(C_{111}^{+--}) = & (1-q^2)^{a/2}\left(1-q-q^2+O(q^4)\right) \\
		e^\RR(C_{111}^{---}) = & (1-q^2)^{a/2}\left(1-3q+3q^2-4q^3  +O(q^4)\right) \\
		e^\RR(C_{111}^{+oo}) = & (1-q^2)^{a/2}\left(1+q+q^2+2q^3  +O(q^4)\right) \\
		e^\RR(C_{111}^{-oo}) = & (1-q^2)^{a/2}\left(1-q+q^2-2q^3  +O(q^4)\right) \\
		\end{align*}
		\end{lem}
		
		\begin{proof}
		
		\end{proof}
	}



\section{Bitangent lines to a planar curve}\label{sec:count}

	\subsection{Setting}
	
	\subsubsection{The surface.} We consider a curve $R$ (as in ``Ramification") of even degree $d$ inside $\CC P^2$. We can consider the double cover of $\CC P^2$ ramified over $R$. This is a complex surface $\CC S$:
	$$\pi:\CC S\longrightarrow \CC P^2.$$
	The Euler characteristic of the latter is given by
	\begin{align*}
	\chi(\CC S) = & 2\chi(\CC P^2)-\chi(\CC R) \\
	= & 6 +d(d-3) .\\ 
	\end{align*}
	
	\subsubsection{The linear system.} The surface is endowed with the line bundle $\L=\pi^*\O(1)$. The curves in the associated linear system $|\L|$ are precisely the lifts of the lines in $\CC P^2$ under the cover.
	
	If the line is transverse to the ramification locus $\CC R$, it has $d$ intersection points with $\CC R$. The corresponding curve in the linear system is a smooth curve having Euler characteristic $4-d$, as it is a double cover of a line ramified at $d$ points.
	
	If the line is not transverse to $\CC R$, the corresponding curve in $\CC S$ acquires a singularity, depending on the tangency order with $\CC R$:
	\begin{itemize}[label=$\ast$]
	\item If the line is tangent to $\CC R$, the curve acquires a node, \textit{i.e.} an $A_1$ singularity.
	\item If the line has intersection index $3$ with $\CC R$, the curve acquires a cusp, \textit{i.e.} an $A_2$ singularity.
	\item If the line is a bitangent to $\CC R$, the curve has two nodes.
	\end{itemize}
	
	\subsubsection{Real structure.} If the curve $R$ is assumed to be real, the complex surface $S$ can also be endowed with a real structure. More precisely, if $R$ is given by a real polynomial $f$ of even degree, and it splits $\RR P^2$ as $\RR P^2_+\sqcup\RR P^2_-$, depending on the sign if $f$. The surface $S$ can be defined by the equation
	$$w^2-f(x,y,z)=0,$$
	in a weighted projective plane. The involution of the ramified covering is $(w,[x:y:z])\mapsto(-w,[x:y:z])$. The two real structures are given by
	$$(w,[x:y:z])\longmapsto (\overline{w},[\overline{x}:\overline{y}:\overline{z}]),$$
	$$(w,[x:y:z])\longmapsto (-\overline{w},[\overline{x}:\overline{y}:\overline{z}]).$$
	The real locus are the lifts of $\RR P^2_+$ and $\RR P^2_-$ by the cover.
	
	We have $\chi(\RR P^2_+)+\chi(\RR P^2_-)=1$.
	
	
	\subsection{Stratification of the discriminant}
	
	\subsubsection{Description and parametrization.} The linear system $|\L|$ of curves in $S$ is isomorphic to the $2$-dimensional projective space. It is in bijection with the space of lines in $\CC P^2$. However, $|\L|$ has more structure as it contains a discriminant $\Delta$ corresponding to singular curves in $S$, \textit{i.e.} to the lines in $\CC P^2$ which are at least tangent to $R$. Thus, the discriminant is parametrized by $R$:
	$$p\in R\longmapsto T_p R.$$
	The map associates to a point $p$ the curve in $|\L|$ corresponding to the tangent to $R$ at $p$.
	
	\subsubsection{Stratification.} The discriminant is stratified according to the type of singularities that the curve acquire:
	\begin{itemize}[label=$\ast$]
	\item The smooth strata $\Delta_1$ corresponding to lines which are tangent to $R$ at a unique point, \textit{i.e.} the curve have a unique node.
	\item The strata $\Delta_2$ corresponding to tangents at an inflection point, \textit{i.e.} the curve has a cusp.
	\item The strata $\Delta_{11}$ corresponding to bitangent.
	\end{itemize}
	The first strata is of dimension $1$ while the other two have dimension $0$. Let $t_\CC$ be the number of bitangents and $i_\CC$ the number of inflection points.
	
	In the real case, we have the real curves and the pairs of complex conjugate curves. Among the bitangents, there are two types: the bitangents at two real points, let $t_2$ be their number, and the bitangents at two complex conjugate points, let $t_0$ be their number. Let also $i$ be the number of real inflection points. The numbers $t_0,t_2,i$ depend on the choice of $R$.
	
	\begin{prop}
	We have the following identity:
	$$\chi(\CC\Delta_1)+i_\CC+2t_\CC=\chi(\CC R).$$
	In the real case, we have the following analog:
	$$\chi(\RR\Delta_1)+2t_2+i=0.$$
	\end{prop}
	
	\begin{proof}
	We have a map $\CC R\to\CC Delta$ which is generically one to one. The only points in $\CC\Delta$ which do not have a unique preimage are bitangents: they have $2$.
	For the real analog, we have a map $\RR R\to\RR\Delta$. The map is also one to one, except at the points corresponding to bitangents at real points. The bitangents at complex conjugate points do not show up in the image since they are not tangent to $\RR R$. In fact, the discriminant is a curve, and complex bitangents correspond to elliptic nodes of the discriminant.
	\end{proof}
	
	
	\subsection{Equations given by the complex Hilbert schemes}
	
	
	
	\subsubsection{First Hilbert scheme.} We consider the universal curve of the linear system and compute its Euler characteristic using the two projections it is endowed with:
	$$\begin{tikzcd}
		 & \CC\CCC \arrow[dl] \arrow[dr] &  \\
		{\CC|\L|} &  & {\CC S} \\
		\end{tikzcd}$$
	
	\begin{prop}
	We have the following identity:
	$$i_\CC=3d(d-2).$$
	\end{prop}
	
	\begin{proof}
	For every point in the surface $\CC S$, there is a pencil of curves passing through it. Thus, we get that
	\begin{align*}
	\chi(\CC\CCC)= & \chi(\CC S)\chi(\CC P^1) \\
	= & 12+2d(d-3) . \\
	\end{align*}
	On the other side, using the computation of the Euler characteristic of the curves appearing in $|\L|$, we have the following:
	\begin{align*}
	\chi(\CC\CCC) = & -a\chi(\CC|\L|) + \chi(\Delta_1)+2t_\CC+2i_\CC \\
	= & -a\chi(\CC P^2) + \chi(\CC R) + i_\CC  \\
	= & 3(4-d)-d(d-3)+i_\CC.\\
	\end{align*}
	The identity follows.
	\end{proof}
	
	
	
	
	\subsubsection{Second Hilbert scheme.} We now use the two pointed relative Hilbert scheme $S^{[2]}$ of the surface $S$, parametrizing length $2$ subschemes of $S$:
	$$\begin{tikzcd}
		 & \CC\CCC^{[2]} \arrow[dl] \arrow[dr] &  \\
		{\CC|\L|} &  & {\CC S^{[2]}} \\
		\end{tikzcd}$$
	
	\begin{prop}
	We have the following identity:
	$$t_\CC=\frac{1}{2}d(d-2)(d+3)(d-3).$$
	\end{prop}
	
	\begin{proof}
	The Hilbert scheme $\CC S^{[2]}$ is stratified as follows:
	\begin{itemize}[label=$\ast$]
	\item We have the length $2$ subschemes corresponding to a pair of distinct points on $S$. Given a pair of distinct points,
		\begin{itemize}[label=-]
		\item If the points have the image in $\CC P^2$, there is a pencil of curves passing through them, since any curve passing through one of them also passes through the other.
		\item If the points have distinct image in $\CC P^2$, a unique curve passes through them: the lift of the unique line passing through their images.
		\end{itemize}
	\item We have the length $2$ subscheme corresponding to a point along with a tangent direction. If the point does not belong to the ramification locus, there is a unique curve containing this length $2$ subscheme: the lift of the line given by the image and the tangent direction. If the point belongs to the ramification locus, we have two possibilities:
		\begin{itemize}[label=-]
		\item If the direction is the kernel of $\mathrm{d}_p\pi$, then every curve in the pencil contains the length $2$ subscheme.
		\item If not, then only the curve coming from the lift of the tangent to $\CC R$ contains the length $2$ subscheme.
		\end{itemize}
	\end{itemize}
	We get the following identity. The first term is for the pairs of distinct points in $\CC S$. The second one is the correction for the pairs of points coming from the involution, which should be counted with multiplicity $\chi(\CC P^1)=2$ instead of $1$. The third term is for points with a tangent direction, that do not belong to the ramification locus, and the last term for the points in the ramification locus, counted with weight the Euler characteristic of the wedge of two spheres: $3$. In the end,
	\begin{align*}
	\chi(\CC\CCC^{[2]}) = & \frac{\chi(\CC S)^2-\chi(\CC S)}{2}+\left(\chi(\CC P^2)-\chi(\CC R)\right)+\left(\chi(\CC S)-\chi(\CC R)\right)\chi(\CC P^1)+3\chi(\CC R) \\
	= & \frac{\chi(\CC S)(\chi(\CC S)+3)}{2}+3 \\
	= & 30 +\frac{15}{2}d(d-3) +\frac{1}{2}d^2(d-3)^2 . \\
	\end{align*}
	
	Now using the second projection and the computation of the Euler characteristic of the $2$-pointed Hilbert scheme, we get that
	\begin{align*}
	\chi(\CC\CCC^{[2]}) = & \bino{a}{2}\chi(\CC|\L|)+(2-a)\chi(\CC\Delta_1)+(4-2a)i_\CC+(5-2a)t_\CC \\
	= & \bino{a}{2}\chi(|\L|)+(2-a)\chi(\CC R)+(2-a)i_\CC+t_\CC \\
	= & \frac{(d-4)(d-5)}{2}\cdot 3 + (d-6)\cdot d(d-3)-(d-6)\cdot 3d(d-2)+t_\CC. \\
	\end{align*}
	
Equating both sides, we get the desired identity.
	\end{proof}
	
	
	
	\subsection{Equations given by the real Hilbert schemes}
	
	\subsubsection{First real Hilbert scheme.} We now consider the real analogs of the complex setting. To obtain a first equation, we consider the complex locus of the real curves in the linear system. We do not consider the real locus of the real curves since it would yield a manifold of dimension $3$, having automatically $0$ as Euler characteristic.
	$$\begin{tikzcd}
		 & \CC\CCC|_{\RR|\L|} \arrow[dl] \arrow[dr] &  \\
		{\RR|\L|} &  & {\CC S} \\
		\end{tikzcd}$$

	We get the following identity that relates the number of complex bitangents to real inflection points.

	\begin{prop}
	Real inflection points and complex bitangents satisfy the following identity:
	$$i+2t_0=d(d-2) .$$
	\end{prop}
	
	\begin{proof}
	We compute the Euler characteristic of $\CC\CCC_{\RR|L|}$ in two ways. First, by integrating over $\CC S$. Given $p\in\CC S$, we have two possibilities:
	\begin{itemize}[label=$\ast$]
	\item If $\pi(p)\notin\RR P^2$, the only real curve passing through $p$ is the lift of the real line passing through $\pi(p)$ and $\overline{\pi(p)}$.
	\item If $\pi(p)\in\RR P^2$, then the lift of any real line passing through $\pi(p)$ yields a curve passing through $p$, and we get a pencil of real lines.
	\end{itemize}
	Moreover, we have that $\chi(\pi^{-1}(\RR P^2)) = 2\chi(\RR P^2)-\chi(\RR\R) = 2$. Therefore, we get that
	\begin{align*}
	\chi(\CC\CCC|_{\RR|\L|} = & \chi(\CC S-\pi^{-1}(\RR P^2))+\chi(\RR P^1)\chi(\pi^{-1}(\RR P^2)) \\
	= & 4+d(d-3).\\
	\end{align*}
	On the other side, using the Euler characteristics of the member of the linear system, we have
	\begin{align*}
	\chi(\CC\CCC|_{\RR|\L|}) = & -a\chi(\RR|\L|) + \chi(\RR\Delta_1)+2t_2+2i+2t_0 \\
	= & (4-d)+i+2t_0.\\
	\end{align*}
	In the end, we get the desired relation.
	\end{proof}
	
	\begin{rem}
	It is possible to obtain the same equation by rather looking at the ramification locus of the real curves in the linear system, which is a $2$-dimensional manifold with a map to $\RR S$.
	\end{rem}
	
	
	
	\subsubsection{Second real Hilbert scheme.} To obtain a second equation, we now consider the real part of the $2$-pointed relative Hilbert scheme of the linear system:
	$$\begin{tikzcd}
		 & \RR\CCC^{[2]} \arrow[dl] \arrow[dr] &  \\
		{\RR|\L|} &  & {\RR S^{[2]}} \\
		\end{tikzcd}$$
		
	Given a real structure on $\CC S$, the real bitangents are of two kinds according to the type of node they induce on the corresponding curve in $\RR|\L|$: they can have two elliptic nodes, two hyperbolic nodes, or one of each. Moreover, changing the real structure on $\CC S$ switches hyperbolic and elliptic nodes. To get numbers not depending on the choice of the real structure on $\CC S$,
	\begin{itemize}[label=$\ast$]
	\item let $t_2^+$ be the number of real bitangents with two hyperbolic or two elliptic nodes,
	\item let $t_2^-$ be the number of real bitangents with an elliptic and an hyperbolic node.
	\end{itemize}
	
	We have the following signed count of bitangents.
		
	\begin{prop}
	The counts of real bitangents satisfy the following relation:
	$$t_2^+ + t_0 - t_2^- = \frac{1}{2}d(d-2)+\frac{1}{2}\chi(\RR S)\left(\chi(\RR S)-2\right) .$$
	\end{prop}
	
	\begin{proof}
	We compute in two ways the Euler characteristic of $\RR\CCC^{[2]}$. To compute it using the map to $\RR S^{[2]}$, we consider the following stratification of $\RR S^{[2]}$: a point of $\RR S^{[2]}$ is of one of the following kinds,
	\begin{itemize}[label=$\ast$]
	\item A pair of distinct real points $(p,q)$. If we have $\pi(p)=\pi(q)$, then we have a pencil of real curves passing through them. Otherwise, we get a unique curve. Thus, this part contributes for
	$$\frac{\chi(\RR S)^2-\chi(\RR S)}{2}-\frac{1}{2}\chi(\RR S).$$
	\item A pair of complex conjugate points $(p,\overline{p})$. If $\pi(p)\notin\RR P^2$, we get a unique curve passing through $p$ and $\overline{p}$. Otherwise, we get a pencil of real curves. Thus, the contribution of this part is
	$$\frac{1}{2}\chi(\CC S-\pi^{-1}(\RR P^2)) = 2+\frac{1}{2}d(d-3).$$
	\item A real point $p$ with a real tangent direction. We have several subcases:
		\begin{itemize}[label=-]
		\item Assume the point does not belong to the ramification locus. Then, for each choice of tangent direction, we get a unique curve which is the lift of the line given by $\pi(p)$ and the image of the tangent direction. As we have a $\RR P^1$ possible choice of tangent directions for each point, the contribution to the Euler characteristic is $0$.
		\item Assume the point belongs to the ramification locus. If the tangent direction is the kernel of $\mathrm{d}_p\pi$, then every curve passing through $p$ contains the given length $2$ subscheme. If not, then only the nodal curve coming from the tangent to $\RR\R$ at $\pi(p)$ contains the given length $2$ subscheme. We get a wedge of two circles, with Euler characteristic $-1$. However, as it needs to be integrated over $\RR\R$, which has Euler characteristic $0$, this part also contributes for $0$.
		\end{itemize}
	\end{itemize}
	In the end, we get that
	$$\chi(\RR\CCC^{[2]}) = \frac{1}{2}\chi(\RR S)\left(\chi(\RR S)-2\right) + 2 +\frac{1}{2}d(d-2).$$	
	We now use the map to $\RR|\L|$ and the computation of the Hilbert schemes. The crucial point is that for curves having two hyperbolic or two elliptic nodes, both have $\chi(\RR C_1^{[2]})=-\frac{a}{2}+1$, while for curves having one of each, $\chi(\RR C_1^{[2]})=-\frac{a}{2}-1$. We get
	\begin{align*}
	\chi(\RR\CCC^{[2]}) = & -\frac{1}{2}a\chi(\RR|\L|) +t_2^{+}+t_0-t_2^{-}.\\
	\end{align*}
	We get the desired identity.
	\end{proof}

	\begin{rem}
	Notice that the quantity $\frac{1}{2}\chi(\RR S)\left(\chi(\RR S)-2\right)$ does not depend on the choice of real structure that we put on $\CC S$.
	\end{rem}
	
	The sign associated to each bitangent is related to the Welschinger sign as it depend on the parity of the number of nodes of a given type.





